Rethinking Deep Thinking: Stable Learning of Algorithms using Lipschitz Constraints

Iterative algorithms solve problems by taking steps until a solution is reached. Models in the form of Deep Thinking (DT) networks have been demonstrated to learn iterative algorithms in a way that can scale to different sized problems at inference time using recurrent computation and convolutions. However, they are often unstable during training, and have no guarantees of convergence/termination at the solution. This paper addresses the problem of instability by analyzing the growth in intermediate representations, allowing us to build models (referred to as Deep Thinking with Lipschitz Constraints (DT-L)) with many fewer parameters and providing more reliable solutions. Additionally our DT-L formulation provides guarantees of convergence of the learned iterative procedure to a unique solution at inference time. We demonstrate DT-L is capable of robustly learning algorithms which extrapolate to harder problems than in the training set. We benchmark on the traveling salesperson problem to evaluate the capabilities of the modified system in an NP-hard problem where DT fails to learn.

==> Sections/analysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis}

\Jay{Analysis of improvements and comparing model structure. Thoughts on
changes.}

\subsection{[IMPACT OF?] Incremental Progress Training}
\Jay{IPT was made to `encourage the system to incrementally make progress
from any starting point'. If our modifications ensure that a system will always
converge to the same fixed point for a given input, then this encouragement
is not required. This part examines to what extent IPT has an impact on
our models.}

We chose to analyze the impact of IPT on prefix sum models with width
\(w=16\).


































































































